SE(3)-Equivariant Relational Rearrangement with Neural Descriptor Fields

We present a method for performing tasks involving spatial relations between novel object instances initialized in arbitrary poses directly from point cloud observations. Our framework provides a scalable way for specifying new tasks using only 5-10 demonstrations. Object rearrangement is formalized as the question of finding actions that configure task-relevant parts of the object in a desired alignment. This formalism is implemented in three steps: assigning a consistent local coordinate frame to the task-relevant object parts, determining the location and orientation of this coordinate frame on unseen object instances, and executing an action that brings these frames into the desired alignment. We overcome the key technical challenge of determining task-relevant local coordinate frames from a few demonstrations by developing an optimization method based on Neural Descriptor Fields (NDFs) and a single annotated 3D keypoint. An energy-based learning scheme to model the joint configuration of the objects that satisfies a desired relational task further improves performance. The method is tested on three multi-object rearrangement tasks in simulation and on a real robot. Project website, videos, and code: https://anthonysimeonov.github.io/r-ndf/

==> figure_text/qual_sim_failures.tex <==
\begin{wrapfigure}{r}{.4\linewidth}
\centering
\vspace{-50pt}
\includegraphics[width=\linewidth]{figures/qual_results_sim.pdf}
\caption{ \small Representative predictions made by each method in simulation experiment}
\vspace{-10pt}
\label{fig:results-common-failures}
\end{wrapfigure}


==> tables/table_ablation.tex <==
\begin{table}[t]
    \centering

\footnotesize
\setlength{\tabcolsep}{2.3pt}
\centering

\begin{tabular}{ccc|cc}
    \toprule
    \textbf{Multiple}  & \textbf{Feature} & \textbf{Learned} & \textbf{Upright} & \textbf{Arbitrary} \\
     \textbf{Demonstration} & \textbf{Alignment} & \textbf{Refinement} & \textbf{Pose} & \textbf{Pose} \\
    \midrule
    No & No & No & 39.3 & 43.6 \\
    Yes & No & No & 66.0 & 60.0\\
    Yes & Yes & No & 80.0 & 72.0 \\
    Yes & Yes & Yes & 84.0  & 75.0 \\
    \bottomrule
\end{tabular}
    
\caption{\small \textbf{Ablations.} Performance of \ourshort with different components ablated. \ourshort without multiple demonstrations operates on a single demonstration. }
 \label{tbl:ablation}

\end{table}

==> tables/table_main.tex <==
\begin{table}
\footnotesize
\setlength{\tabcolsep}{2.3pt}
\centering
\begin{tabular}{@{}lcccccc@{}}
    \toprule
      & \multicolumn{2}{c}{\textbf{Bowl on Mug}} & \multicolumn{2}{c}{\textbf{Mug on Rack}} & \multicolumn{2}{c}{\textbf{Bottle in Container}}  \\
     \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} 
     \textbf{Method} & Upright &  Arbitrary & Upright & Arbitrary &  Upright & Arbitrary \\
     \midrule
       Pose Regression & 35.0 & 6.0 & 13.0 & 10.0 & 37.9 & 12.0 \\
       Patch Match & 34.0 & 32.0 & 56.0 & 44.0 & 44.0 & 42.0 \\
      \ourshort & 74.0 & 70.0 & 84.0 & 75.0 & 80.0 & 75.0 \\
    \bottomrule
    
\end{tabular}
\vspace{5pt}
\caption{\small \textbf{Relation inference success rates in simulation.} \ourshort works better than all other approaches.}
\label{tbl:benchmark}
\vspace{-20pt}
\end{table}

==> text/problem_setup.tex <==
\section{Demonstration and Task Setup}
\label{sec:problem-setup}
Our setup consists of a robot in a quasistatic tabletop environment with a rigid ``parent'' object and ``child'' object. \pulkit{Using parent and child gives a notion that the "child" is a subset of the parent, like in a graph how the parent node subdivides into children. Maybe just call object A and B or some other names? Maybe given an example -- mug hanging on the rack -- mug is object A, rack is object B.} % \asnote{notation for demo object vs. test-time object?}
%
The goal is to allow a user to specify some geometric relationship between the parent and child via a small set of demonstrations. 
%
Examples of relations we consider include ``\emph{mug hanging by its handle on the peg of a rack}'', ``\emph{bowl placed upright on top of a mug}'', and ``\emph{bottle placed upright in the corner of a tray}''. 

\myparagraph{Demonstration Setup}
%
When collecting a demonstration $\mathcal{D}$, we obtain an initial segmented 3D point cloud ($\demopointcloud_{p} \in \mathbb{R}^{N \times 3}$ and $\demopointcloud_{c} \in \mathbb{R}^{N \times 3}$) of the parent and child objects ($\demoobject_{p}$ and $\demoobject{c}$).
%
The demonstrator then moves the objects into their final configuration, while recording each rigid body transformation that is applied to each object.
%
The overall transformation that brings each object into its final configuration is represented as a single \sethree{} transformation $\demopose_{p} = (\hat{\mathbf{R}}_{p}, \hat{\mathbf{t}}_{p})$ and $\demopose_{c} = (\hat{\mathbf{R}}_{c}, \hat{\mathbf{t}}_{c})$, from which we obtain final transformed point clouds $\demopointcloud^{f}_{p}$ = $\hat{\mathbf{R}}_{p}\demopointcloud_{p} + \hat{\mathbf{t}}_{p}$ and $\demopointcloud^{f}_{c}$ = $\hat{\mathbf{R}}_{c}\demopointcloud_{c} + \hat{\mathbf{t}}_{c}$. Throughout this paper we will typically assume an the parent object transformation $\demopose_{p}$ is the identity transformation
, such that $\demopointcloud_{p} = \demopointcloud^{f}_{p}$.  

\myparagraph{Test-time Task Setup}
At test time, we are given a new parent and child object ($\object_{p}$ and $\object_{c}$), each with potentially new shapes and poses.
%
We assume the system has access to a segmented point cloud of each object, $\pointcloud^{s}_{p}$ and $\pointcloud^{s}_{c}$, and knows the identify of the parent and child.
%
The task is to use these point cloud observations and the $K$ demonstrations $\{\mathcal{D}_{i}\}_{i=1}^{K}$ to infer a relative transformation of the child object $\pose_{c}$.
%
$\pose_{c}$ is applied to $\object_{c}$ by performing a pick-and-place action with the robot, where an initial grasp pose $\pose_{\text{grasp}}$ (obtained using a separate grasp generation pipeline) is transformed by $\pose_{c}$ to obtain a placing pose $\pose_{\text{place}} = \pose_{c}\pose_{\text{grasp}}$.
%
After releasing the child object in the final configuration, task success is determined based on if $\object_{c}$ and $\object_{p}$ satisfy the same geometric relation that was specified in the demonstrations. % \asnote{We are missing a formal explanation that we could also consider a transformation of the parent object to bring it into it's own stable + upright pose. Will circle back around and add this}. 
